Learning Deep Representations Using Convolutional Auto-encoders with Symmetric Skip Connections

Unsupervised pre-training was a critical technique for training deep neural networks years ago. With sufficient labeled data and modern training techniques, it is possible to train very deep neural networks from scratch in a purely supervised manner nowadays. However, unlabeled data is easier to obtain and usually of very large scale. How to make use of them better to help supervised learning is still a well-valued topic. In this paper, we investigate convolutional denoising auto-encoders to show that unsupervised pre-training can still improve the performance of high-level image related tasks such as image classification and semantic segmentation. The architecture we use is a convolutional auto-encoder network with symmetric shortcut connections. We empirically show that symmetric shortcut connections are very important for learning abstract representations via image reconstruction. When no extra unlabeled data are available, unsupervised pre-training with our network can regularize the supervised training and therefore lead to better generalization performance. With the help of unsupervised pre-training, our method achieves very competitive results in image classification using very simple all-convolution networks. When labeled data are limited but extra unlabeled data are available, our method achieves good results in several semi-supervised learning tasks.

==> figures/loss.tex <==
%\begin{figure}[]
%    \begin{subfigure}[normal]{0.5\linewidth}
%    \centering
%        \includegraphics[scale=0.5]{figures/loss/cifar10}
%        \caption{CIFAR-10}
%    \end{subfigure}%
%    \begin{subfigure}[normal]{0.5\linewidth}
%        \includegraphics[scale=0.5]{figures/loss/cifar100}
%        \caption{CIFAR-100}
%    \end{subfigure}%
%    \caption{Training loss on first 50 epochs using different initialization methods.}
%    \label{fig:loss}
%\end{figure}

\begin{figure}[]
    \begin{subfigure}[normal]{\linewidth}
        \centering
        \includegraphics[scale=0.5]{figures/loss/cifar10}
    \end{subfigure}
    \caption{Training loss at first 50 epochs using different initialization methods on CIFAR-10}
    \label{fig:loss}
\end{figure}

==> figures/stl10.tex <==
\begin{figure}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figures/stl10.png}

    \caption{STL-10 testing accuracy on different number of labeled images.}
    \label{fig:stl10_label}
\end{figure}

==> tables/architecture.tex <==
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|}
\hline
             & Network-1     & Network-2     \\ \hline
block 1      & \begin{tabular}[c]{@{}c@{}}conv 3x3,n\\ ...\\ $\times(m_1-1)$\end{tabular}       & conv 3x3,64                                                               \\ \hline
downsample 1 & conv 3x3/2, n                                                             & conv 3x3/2,64                                                             \\ \hline
block 2      & \begin{tabular}[c]{@{}c@{}}conv 3x3,2n\\ ...\\ $\times(m_2-1)$\end{tabular}      & conv 3x3,128                                                              \\ \hline
downsample 2 & conv 3x3/2,2n                                                             & conv 3x3/2,128                                                            \\ \hline
block 3      & \begin{tabular}[c]{@{}c@{}}conv 3x3,4n\\ ...\\ $\times(m_3-1)$\end{tabular}      & \begin{tabular}[c]{@{}c@{}}conv 3x3, 256\\ conv 3x3, 256\end{tabular}     \\ \hline
downsample 3 & conv 3x3/2,4n                                                             & conv 3x3/2, 256                                                           \\ \hline
block 4      & \begin{tabular}[c]{@{}c@{}}conv 3x3,8n\\ ...\\ $\times(m_4-1)$\end{tabular}    & \begin{tabular}[c]{@{}c@{}}conv 3x3, 512\\ conv 3x3, 512\end{tabular}     \\ \hline
downsample 4 & conv 3x3/2,8n                                                             & conv 3x3/2, 512                                                           \\ \hline
block 5      &                                                                           & \begin{tabular}[c]{@{}c@{}}conv 3x3, 512\\ conv 3x3, 512\end{tabular}     \\ \hline
downsample 5 &                                                                           & conv 3x3/2, 512                                                           \\ \hline
block 6        & \begin{tabular}[c]{@{}c@{}}global\_ave\_pool\\ fc,num\_class\end{tabular} & \begin{tabular}[c]{@{}c@{}}fc,4096\\ fc,4096\\ fc,num\_class\end{tabular} \\ \hline
\end{tabular}
\caption{Network architectures. Network-1 is used for CIFAR-10, CIFAR-100 and STL-10. Network-2 is based on VGG-16 and used for PASCAL VOC. }
\label{table:architecture}
\end{table}

==> tables/cifar_100_state.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|}
\hline
Method                        &Accuracy  \\ \hline
Spatially-sparse                        &75.7\%   \\ \hline
ELU                                     &75.72\%   \\ \hline
Fractional Max-Pooling                  &73.61\%   \\ \hline
Resnet-v1-164 \cite{resnet}            &74.84\%   \\ \hline
Resnet-v1-1001 \cite{resnet}           &72.18\%   \\ \hline
Resnet-v2-164 \cite{new_resnet}        &75.67\%   \\ \hline
Resnet-v2-1001 \cite{new_resnet}       &77.29\%   \\ \hline
Ours 15-128-random                      &73.62\%    \\ \hline
Ours 15-128-cifar10                     &75.68\%   \\ \hline
Ours 15-128-cifar100                    &75.41\%   \\ \hline

\end{tabular}
\caption{Comparisons with state-of-the-arts: CIFAR-100 classification accuracy (with simple data-augmentation).}
\label{table:cifar_100_state}
\end{table}

==> tables/cifar_10_state.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|}
\hline
Method                         &Accuracy  \\ \hline
All-conv-net \cite{all_conv}            &92.75\%   \\ \hline
%Resnet-20 \cite{resnet}                 &91.25\%   \\ \hline
Resnet-164 \cite{resnet}                &93.57\%   \\ \hline
Resnet-new-164 \cite{new_resnet}        &93.57\%   \\ \hline
Resnet-new-1001 \cite{new_resnet}       &95.08\%   \\ \hline
Resnet-new-1001 \cite{new_resnet}       &95.38\%   \\ \hline
Ours 10-64                              &93.31\%   \\ \hline
Ours 15-64                              &94.14\%   \\ \hline
Ours 15-128                             &95.20\%   \\ \hline

\end{tabular}
\caption{Comparisons with state-of-the-arts: CIFAR-10 classification accuracy (with simple data-augmentation).}
\label{table:cifar_10_state}
\end{table}

==> tables/class_compare.tex <==
\begin{table*}[htbp]
\centering
\scalebox{0.5}{
\begin{tabular}{|c|cccccc|ccccccc|cccccc|c|c|}
\hline
\multirow{2}{*}{Init} & \multicolumn{6}{c|}{Animal}                                                                                     & \multicolumn{7}{c|}{Vehicle}                                                                                                       & \multicolumn{6}{c|}{Indoor}                                                                                     & person           & Total            \\ \cline{2-22} 
                      & bird             & cat              & cow              & dog              & horse            & sheep            & plane            & bike             & boat             & bus              & car              & moto             & train            & bottle           & chair            & table            & plant            & sofa             & tv               & -                & -                \\ \hline
Gaussian              & 52.10\%          & 59.41\%          & 39.52\%          & 48.47\%          & 76.39\%          & 42.14\%          & 77.94\%          & 64.28\%          & 59.34\%          & 62.29\%          & 79.05\%          & 72.09\%          & 80.01\%          & 18.71\%          & 49.64\%          & 47.72\%          & 33.72\%          & 50.24\%          & 49.64\%          & 87.15\%          & 57.47\%          \\
Animal                & \textbf{64.53\%} & \textbf{69.15\%} & 51.09\%          & \textbf{61.63\%} & \textbf{81.79\%} & \textbf{51.87\%} & \textbf{80.24\%} & 72.42\%          & 67.03\%          & 62.26\%          & 83.75\%          & \textbf{77.48\%} & 83.15\%          & 25.76\%          & 53.09\%          & 58.21\%          & 41.21\%          & \textbf{61.18\%} & 56.00\%          & 88.98\%          & 64.54\%          \\
Vehicle               & 59.98\%          & 67.93\%          & \textbf{51.89\%} & 59.90\%          & 81.58\%          & 47.27\%          & 80.06\%          & \textbf{74.21\%} & \textbf{71.02\%} & \textbf{65.54\%} & \textbf{85.00\%} & 77.08\%          & \textbf{84.25\%} & \textbf{27.47\%} & \textbf{55.67\%} & \textbf{60.18\%} & \textbf{42.29\%} & 58.79\%          & \textbf{58.42\%} & \textbf{89.18\%} & \textbf{64.89\%} \\ \hline
\end{tabular}
}
\caption{}
\label{my-label}
\end{table*}

==> tables/class_compare_short.tex <==
\begin{table*}[htbp]
\centering
\scalebox{0.7}{
\begin{tabular}{|c|cccccc|ccccccc|cccccc|c|c|}
\hline
\multirow{2}{*}{Data} & \multicolumn{6}{c|}{Animal}                                                                                     & \multicolumn{7}{c|}{Vehicle}                                                                                                       & \multicolumn{6}{c|}{Indoor}                                                                                     & person           & mAP            \\ \cline{2-22} 
                      & bird             & cat              & cow              & dog              & horse            & sheep            & plane            & bike             & boat             & bus              & car              & moto             & train            & bottle           & chair            & table            & plant            & sofa             & tv               & -                & -                \\ \hline
Gaussian              & 52.1         & 59.4          & 39.5          & 48.5          & 76.4          & 42.1          & 77.9          & 64.3          & 59.3          & 62.3          & 79.1          & 72.1          & 80.0          & 18.7          & 49.6          & 47.7          & 33.7          & 50.2          & 49.6          & 87.2          & 57.5          \\
Animal                & \textbf{64.5} & \textbf{69.2} & 51.1          & \textbf{61.6} & \textbf{81.8} & \textbf{51.9} & \textbf{80.2} & 72.4          & 67.0          & 62.3          & 83.8          & \textbf{77.5} & 83.2          & 25.8          & 53.1          & 58.2          & 41.2          & \textbf{61.2} & 56.0          & 89.0          & 64.5          \\
Vehicle               & 60.0          & 67.9          & \textbf{51.9} & 59.9          & 81.6          & 47.3          & 80.1          & \textbf{74.2} & \textbf{71.0} & \textbf{65.5} & \textbf{85.0} & 77.1          & \textbf{84.3} & \textbf{27.5} & \textbf{55.7} & \textbf{60.2} & \textbf{42.3} & 58.8          & \textbf{58.4} & \textbf{89.2} & \textbf{64.9} \\ \hline
\end{tabular}
}
\caption{Compare different pre-training data: Average precision of PASCAL VOC 2007 classification. The animal pre-trained network outperforms on ralated animal classes, so do vehicle pre-trained. All of them are better than the nettwork without pre-training. The pre-training is totally unsupervised.}
\label{table:class_compare}
\end{table*}

==> tables/corruptions.tex <==
\begin{table}[htb!]
\centering
\begin{tabular}{|c|c|c|}
\hline
Corruption                     & \begin{tabular}[c]{@{}c@{}}Data driven\\ initialization\end{tabular} & \begin{tabular}[c]{@{}c@{}}Unsupervised\\ pre-training\end{tabular} \\ \hline
No pre-training         & \multicolumn{2}{c|}{67.11\%}                                                                                                                                       \\ \hline
Pixel Gaussian noise & 68.20\%                                                                 & 69.23\%                                                                                  \\
Patch Gaussian noise & 69.44\%                                                                 & 68.24\%                                                                                  \\
Big missing block    & 68.25\%                                                                &  69.08\%                                                                                  \\
Small missing blocks & \textbf{69.87\%}                                                        & \textbf{71.25\%}                                                                         \\ \hline
\end{tabular}
\caption{Compare different types of corruption: mAP for PASCAL VOC 2007 classification.}
\label{table:corruptions}
\end{table}

==> tables/large_init_compare.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|}
\hline
Initialization                   &mAP  \\ \hline
Random                           &57.62\%   \\ \hline
He \etal~\cite{msra_init}        &     \\ \hline
Xavior \cite{xavier}             &     \\ \hline
Kr{\"{a}}henb{\"{u}}hl \cite{dependent_init}                               &          \\  \hline
Ours Gaussian pixel              &58.04\%   \\ \hline
Ours Gaussian patch              &\textbf{59.2\%}   \\ \hline
Ours Inpainting                  &58.78\%   \\ \hline

\end{tabular}
\caption{Compare with other initialization: PASCAL VOC 2007 classification results}
\label{table:large_init_compare}
\end{table}

==> tables/segmentation.tex <==
\begin{table}[htb!]
\centering
\begin{tabular}{|c|c|}
\hline
Reused Layers         & mean IU \\ \hline
Random Gaussian       & 27.39\% \\
Pre-trained Encoder + random decoder               & 35.85\% \\
Pre-trained Encoder and decoder   & \textbf{39.63\%} \\ \hline
\end{tabular}
\caption{Mean IUs of PASCAL VOC 2012 Segmentation task on validation data with different fine-tuning strategies.}
\label{table:segmentation}
\end{table}

==> tables/shortcut_compare.tex <==
\begin{table}[htb!]
\centering
\begin{tabular}{|c|c|c|}
\hline
              & PSNR  & mAP     \\ \hline
No shortcut   & 22.19 & 68.94\% \\
Input output shortcut & 23.50 & 69.38\% \\
Ours full shortcut & \textbf{23.87} & \textbf{71.25\%} \\ \hline
\end{tabular}
\caption{Comparions of different shortcut strategies on reconstruction PSNR and classification performance after fine-tuning.}
\label{table:shortcut_compare}
\end{table}

==> tables/tiny_init.tex <==
\begin{table}[]
\centering
\begin{tabular}{|c|cc|cc|}
\hline
\multirow{2}{*}{network} & \multicolumn{2}{c|}{CIFAR-10} & \multicolumn{2}{c|}{CIFAR-100} \\ \cline{2-5} 
 & \multicolumn{1}{c|}{random} & ours & \multicolumn{1}{c|}{random} & ours \\ \hline
10-64 & 92.62\% & 93.31\% & - & - \\
15-64 & 93.42\% & 94.14\% & - & - \\
15-128 & 93.95\% & \textbf{94.93\%} & 73.89\% & \textbf{75.41\%} \\ \hline
\end{tabular}
\caption{Compare different architectures: CIFAR-10 and CIFAR-100 classification accuracy}
\label{table:tiny_init}
\end{table}

==> tables/tiny_init_compare.tex <==
\begin{table}[htb!]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
                            & CIFAR-10                  & CIFAR-100          & VOC 2007 \\ \hline
Gaussian                    & 93.95\%                   & 73.89\%            & 67.11\% \\
He \etal~\cite{msra_init}   & 93.67\%                   & 72.15\%            & 66.71\% \\
Xavior\cite{xavier}         & 93.60\%                   & 72.9\%             & 67.27\% \\
%Kr{\"{a}}henb{\"{u}}hl\cite{dependent_init} &  &  \\
Ours                        & \textbf{94.93\%}          & \textbf{75.41\%}   & \textbf{69.87\%} \\ \hline
\end{tabular}
\caption{Comparisons with other initialization methods: CIFAR-10, CIFAR-100 and PASCAL VOC 2007 classification results.}
\label{table:tiny_init_compare}
\end{table}
